Revisiting Reachability in Timed Automata

We revisit a fundamental result in real-time verification, namely that the binary reachability relation between configurations of a given timed automaton is definable in linear arithmetic over the integers and reals. In this paper we give a new and simpler proof of this result, building on the well-known reachability analysis of timed automata involving difference bound matrices. Using this new proof, we give an exponential-space procedure for model checking the reachability fragment of the logic parametric TCTL. Finally we show that the latter problem is NEXPTIME-hard.

==> z0.tex <==
 \begin{tikzpicture}
    \draw[very thin,color=gray,step=.25cm] (0,0) grid (1.25,1.25);    
    \draw[->,thick] (0,0) -- (1.35,0);
    \draw[->,thick] (0,0) -- (0,1.35);

\fill[red!80] (.75,0) circle[radius=2pt];
\end{tikzpicture}

==> z1.tex <==
 \begin{tikzpicture}
    \draw[very thin,color=gray,step=.25cm] (0,0) grid (1.25,1.25);    
    \draw[->,thick] (0,0) -- (1.35,0);
    \draw[->,thick] (0,0) -- (0,1.35);

\draw[-,line width=2pt,blue]  (.75,0)--(1.25,.5);

\end{tikzpicture}

==> z2.tex <==
 \begin{tikzpicture}
    \draw[very thin,color=gray,step=.25cm] (0,0) grid (1.25,1.25);    
    \draw[->,thick] (0,0) -- (1.35,0);
    \draw[->,thick] (0,0) -- (0,1.35);

%\fill[green!80] (0,.625) circle[radius=2pt];
\draw[-,line width=2pt,green]  (0,0)--(0,.5);
\end{tikzpicture}

==> z3ax.tex <==
 \begin{tikzpicture}
    \draw[very thin,color=gray,step=.25cm] (0,0) grid (1.25,1.25);    
    \draw[->,thick] (0,0) -- (1.35,0) node[right] {$x_1$};
    \draw[->,thick] (0,0) -- (0,1.35) node[left] {$x_2$};

\draw [draw=magenta, fill=magenta]
     (0,.375)--  (.875,1.25) -- (.625,1.25) -- (0,.625);
		    \draw[->,thick] (0,0) -- (1.35,0);
    \draw[->,thick] (0,0) -- (0,1.35);
\end{tikzpicture}

==> z4.tex <==
 \begin{tikzpicture}
    \draw[very thin,color=gray,step=.25cm] (0,0) grid (1.25,1.25);    
    \draw[->,thick] (0,0) -- (1.35,0);
    \draw[->,thick] (0,0) -- (0,1.35);


\draw[-,line width=2pt,yellow!10!orange]  (0.625,0)--(1.25,0);
\end{tikzpicture}

==> z5.tex <==
 \begin{tikzpicture}
    \draw[very thin,color=gray,step=.25cm] (0,0) grid (1.25,1.25);    
  
%\draw[-,very thick,cyan]  (.625,0)--(1.25,.625);

\draw [draw=pink, fill=pink]
    (0.625,0)--  (1.25,0) -- (1.25,.5) -- (.625,0);
		  \draw[->,thick] (0,0) -- (1.35,0);
    \draw[->,thick] (0,0) -- (0,1.35);

\end{tikzpicture}
